Double Equivariance for Inductive Link Prediction for Both New Nodes and New Relation Types

The task of fully inductive link prediction in knowledge graphs has gained significant attention, with various graph neural networks being proposed to address it. This task presents greater challenges than traditional inductive link prediction tasks with only new nodes, as models must be capable of zero-shot generalization to both unseen nodes and unseen relation types in the inference graph. Despite the development of novel models, a unifying theoretical understanding of their success remains elusive, and the limitations of these methods are not well-studied. In this work, we introduce the concept of double permutation-equivariant representations and demonstrate its necessity for effective performance in this task. We show that many existing models, despite their diverse architectural designs, conform to this framework. However, we also identify inherent limitations in double permutation-equivariant representations, which restrict these models's ability to learn effectively on datasets with varying characteristics. Our findings suggest that while double equivariance is necessary for meta-learning across knowledge graphs from different domains, it is not sufficient. There remains a fundamental gap between double permutation-equivariant models and the concept of foundation models designed to learn patterns across all domains.

==> src/appdx-additional-example.tex <==
\section{Additional Example for \OurTask}
\label{appd:add-example}

\begin{wrapfigure}{r}{0.55\textwidth}
\centering
%
\includegraphics[width=\linewidth]{figs/alien.drawio.pdf}
%
\caption{
{\bf Alien \ourgraph:}
The task is to predict the missing relation ``?'' in red.
Training only tells us that relations do not repeat in a path.}
\label{fig:example-guess}
%
\end{wrapfigure}
This example depicts an even harder scenario than the example in 
\Cref{fig:example-link}, obtained from a fictional alien civilization.
Knowing nothing about alien languages, we note that in training, all adjacent relations are different. Minimally, we could predict the missing relation in red in test data is not ``$\nless$''. By introducing equivariance in relations, it is possible for a model to predict relation types uniformly over the set of other ($R\!-\!1$) relations except for the existing relation ``$\nless$'', which is all we know about the aliens.  
%


==> src/appdx-future-work.tex <==
\section{Future Work}
\label{sec:sup_future}

As addressed in the main paper, our implemented architecture has a few limitations, which could be addressed in future work.
First, ISDEA+ has high pre-processing cost. This high time cost is introduced by using shortest distances whose computation is of the same complexity as enclosed subgraph. However, our ablation studies show that shortest distances is not a dominant factor in our model for real-world tasks, thus it is possible that shortest distances can be replaced by other heuristics that can be efficiently extracted.

Second, our specific implementation ISDEA happens to have high training and inference costs, since it relies on repeating GNNs for each relation. Thus, complexity ISDEA of scales linearly w.r.t.\ number of relations, which is often a large number in real-world knowledge base, e.g., Wikipedia. However, fully equivariance over all relations can be too strong, and we may only want partial equivariance which may reduce the cost. We resolve this issue by introduing \OurNewModel.

Third, ISDEA+ has expressivity limitation. This limitation is related to former two cost issues since it is caused by compromising most-expressive pairwise representation to node-wise representation due to time cost. Thus if we can reduce the cost, we may be able to use more expressive graph encoder.

Finally, although we show ISDEA+ representations can capture UQER Horn clauses, there is no algorithm to create UQER Horn clauses from ISDEA+ representations. This topic is known as {\em explainability} which is important in graph machine learning community. We leave such an algorithm as another future work other than optimization. 

